The light CP-even MSSM Higgs mass resummed to fourth logarithmic order

We present the calculation of the light neutral CP-even Higgs mass in the MSSM for a heavy SUSY spectrum by resumming enhanced terms through fourth logarithmic order (N$^3$LL), keeping terms of leading order in the top Yukawa coupling $\alpha_t$, and NNLO in the strong coupling $\alpha_s$. To this goal, the three-loop matching coefficient for the quartic Higgs coupling of the SM to the MSSM is derived to order $\alpha_t^2\alpha_s^2$ by comparing the perturbative EFT to the fixed-order expression for the Higgs mass. The new matching coefficient is made available through an updated version of the program Himalaya. Numerical effects of the higher-order resummation are studied using specific examples, and sources of theoretical uncertainty on this result are discussed.

==> biblio.tex <==
%\cite{Stockinger:2018oxe}
\bibitem{Stockinger:2018oxe}
  D.~St\"ockinger and J.~Unger,
  %``Three-loop MSSM Higgs-boson mass predictions and regularization by dimensional reduction,''
  Nucl.\ Phys.\ B {\bf 935} (2018) 1
%  doi:10.1016/j.nuclphysb.2018.08.005
  [arXiv:1804.05619 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2018.08.005;%%
  %3 citations counted in INSPIRE as of 23 Oct 2018
%\cite{Draper:2013oza}
\bibitem{Draper:2013oza}
  P.~Draper, G.~Lee and C.E.M.~Wagner,
  %``Precise estimates of the Higgs mass in heavy supersymmetry,''
  Phys.\ Rev.\ D {\bf 89} (2014) no.5,  055023
  [arXiv:1312.5743 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.055023;%%
  %94 citations counted in INSPIRE as of 18 Sep 2018
%\cite{Hahn:2013ria}
\bibitem{Hahn:2013ria}
  T.~Hahn, S.~Heinemeyer, W.~Hollik, H.~Rzehak and G.~Weiglein,
  %``High-Precision Predictions for the Light CP -Even Higgs Boson Mass of the Minimal Supersymmetric Standard Model,''
  Phys.\ Rev.\ Lett.\  {\bf 112} (2014) no.14,  141801
  [arXiv:1312.4937 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.112.141801;%%
  %261 citations counted in INSPIRE as of 18 Sep 2018
  %
% DO NOT EDIT THIS FILE!
%
% It is generated automatically.
%
% mh3lmatch_ref.tex -- generated by sortref-2.5  
% ((C) R. Harlander, http://www.robert-harlander.de/software/)
% on Thu Aug 23 13:28:37 CEST 2018
%

% (deleting this header may lead to severe nose bleeding)
%

%1
\bibitem{Aad:2015zhl}
  G.~Aad {\it et al.} [ATLAS and CMS Collaborations],
  Phys.\ Rev.\ Lett.\  {\bf 114} (2015) 191803
  [arXiv:1503.07589 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.114.191803;%%

%2
\bibitem{Haber:1990aw}
  H.E.~Haber and R.~Hempfling,
  Phys.\ Rev.\ Lett.\  {\bf 66} (1991) 1815.
  %%CITATION = doi:10.1103/PhysRevLett.66.1815;%%

%3
\bibitem{Okada:1990vk}
  Y.~Okada, M.~Yamaguchi and T.~Yanagida,
  Prog.\ Theor.\ Phys.\  {\bf 85} (1991) 1.
  %%CITATION = doi:10.1143/ptp/85.1.1;%%

%4
\bibitem{Ellis:1990nz}
  J.R.~Ellis, G.~Ridolfi and F.~Zwirner,
  Phys.\ Lett.\ B {\bf 257} (1991) 83.
  %%CITATION = doi:10.1016/0370-2693(91)90863-L;%%

%5
\bibitem{Ellis:1991zd}
  J.R.~Ellis, G.~Ridolfi and F.~Zwirner,
  Phys.\ Lett.\ B {\bf 262} (1991) 477.
  %%CITATION = doi:10.1016/0370-2693(91)90626-2;%%

%6
\bibitem{Barbieri:1991tk}
  R.~Barbieri and M.~Frigeni,
  Phys.\ Lett.\ B {\bf 258} (1991) 395.
  %%CITATION = doi:10.1016/0370-2693(91)91106-6;%%

%7
\bibitem{Chankowski:1992er}
  P.H.~Chankowski, S.~Pokorski and J.~Rosiek,
  Nucl.\ Phys.\ B {\bf 423} (1994) 437
  [hep-ph/9303309].
  %%CITATION = doi:10.1016/0550-3213(94)90141-4;%%

%8
\bibitem{Dabelstein:1994hb}
  A.~Dabelstein,
  Z.\ Phys.\ C {\bf 67} (1995) 495
  [hep-ph/9409375].
  %%CITATION = doi:10.1007/BF01624592;%%

%9
\bibitem{Allanach:2004rh}
  B.C.~Allanach, A.~Djouadi, J.L.~Kneur, W.~Porod and P.~Slavich,
  JHEP {\bf 0409} (2004) 044
  [hep-ph/0406166].
  %%CITATION = doi:10.1088/1126-6708/2004/09/044;%%

%10
\bibitem{Bagnaschi:2014rsa}
  E.~Bagnaschi, G.F.~Giudice, P.~Slavich and A.~Strumia,
  JHEP {\bf 1409} (2014) 092
  [arXiv:1407.4081 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP09(2014)092;%%

%11
\bibitem{Vega:2015fna}
  J.~Pardo Vega and G.~Villadoro,
  JHEP {\bf 1507} (2015) 159
  [arXiv:1504.05200 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2015)159;%%

%12
\bibitem{Bahl:2016brp}
  H.~Bahl and W.~Hollik,
  Eur.\ Phys.\ J.\ C {\bf 76} (2016) no.9,  499
  [arXiv:1608.01880 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-016-4354-8;%%

%13
\bibitem{Bahl:2017aev}
  H.~Bahl, S.~Heinemeyer, W.~Hollik and G.~Weiglein,
  Eur.\ Phys.\ J.\ C {\bf 78} (2018) no.1,  57
  [arXiv:1706.00346 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-018-5544-3;%%

%14
\bibitem{Allanach:2018fif}
  B.C.~Allanach and A.~Voigt,
  Eur.\ Phys.\ J.\ C {\bf 78} (2018) no.7,  573
  [arXiv:1804.09410 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-018-6046-z;%%

%15
\bibitem{Bagnaschi:2017xid}
  E.~Bagnaschi, J.~Pardo Vega and P.~Slavich,
  Eur.\ Phys.\ J.\ C {\bf 77} (2017) no.5,  334
  [arXiv:1703.08166 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-4885-7;%%

%16
\bibitem{Athron:2017fvs}
  P.~Athron, M.~Bach, D.~Harries, T.~Kwasnitza, J.h.~Park,
  D.~St\"ockinger, A.~Voigt and J.~Ziebell, Comput.\ Phys.\ Commun.\
  {\bf 230} (2018) 145 [arXiv:1710.03760 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2018.04.016;%%

%17
\bibitem{Athron:2016fuq}
  P.~Athron, J.~h.~Park, T.~Steudtner, D.~St\"ockinger and A.~Voigt,
  JHEP {\bf 1701} (2017) 079
  [arXiv:1609.00371 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2017)079;%%

%18
\bibitem{Staub:2017jnp}
  F.~Staub and W.~Porod,
  Eur.\ Phys.\ J.\ C {\bf 77} (2017) no.5,  338
  [arXiv:1703.03267 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-4893-7;%%

%19
\bibitem{Bahl:2018jom}
  H.~Bahl and W.~Hollik,
  JHEP {\bf 1807} (2018) 182
  [arXiv:1805.00867 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2018)182;%%

%20
\bibitem{Athron:2014yba}
  P.~Athron, J.~h.~Park, D.~St\"ockinger and A.~Voigt,
  Comput.\ Phys.\ Commun.\  {\bf 190} (2015) 139
  [arXiv:1406.2319 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2014.12.020;%%

%21
\bibitem{Porod:2003um}
  W.~Porod,
  Comput.\ Phys.\ Commun.\  {\bf 153} (2003) 275
  [hep-ph/0301101].
  %%CITATION = doi:10.1016/S0010-4655(03)00222-4;%%

%22
\bibitem{Staub:2009bi}
  F.~Staub,
  Comput.\ Phys.\ Commun.\  {\bf 181} (2010) 1077
  [arXiv:0909.2863 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2010.01.011;%%

%23
\bibitem{Porod:2011nf}
  W.~Porod and F.~Staub,
  Comput.\ Phys.\ Commun.\  {\bf 183} (2012) 2458
  [arXiv:1104.1573 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2012.05.021;%%

%24
\bibitem{Staub:2010jh}
  F.~Staub,
  Comput.\ Phys.\ Commun.\  {\bf 182} (2011) 808
  [arXiv:1002.0840 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2010.11.030;%%

%25
\bibitem{Staub:2012pb}
  F.~Staub,
  Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 1792
  [arXiv:1207.0906 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2013.02.019;%%

%26
\bibitem{Staub:2013tta}
  F.~Staub,
  Comput.\ Phys.\ Commun.\  {\bf 185} (2014) 1773
  [arXiv:1309.7223 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2014.02.018;%%

%27
\bibitem{Allanach:2001kg}
  B.C.~Allanach,
  Comput.\ Phys.\ Commun.\  {\bf 143} (2002) 305
  [hep-ph/0104145].
  %%CITATION = doi:10.1016/S0010-4655(01)00460-X;%%

%28
\bibitem{Allanach:2014nba}
  B.C.~Allanach, A.~Bednyakov and R.~Ruiz de Austri,
  Comput.\ Phys.\ Commun.\  {\bf 189} (2015) 192
  [arXiv:1407.6130 [hep-ph]].
  %%CITATION = doi:10.1016/j.cpc.2014.12.006;%%

%29
\bibitem{Djouadi:2002ze}
  A.~Djouadi, J.L.~Kneur and G.~Moultaka,
  Comput.\ Phys.\ Commun.\  {\bf 176} (2007) 426
  [hep-ph/0211331].
  %%CITATION = doi:10.1016/j.cpc.2006.11.009;%%

%30
\bibitem{Bednyakov:2013eba}
  A.V.~Bednyakov, A.F.~Pikelner and V.N.~Velizhanin,
  Nucl.\ Phys.\ B {\bf 875} (2013) 552
  [arXiv:1303.4364 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2013.07.015;%%

%31
\bibitem{Harlander:2008ju}
  R.V.~Harlander, P.~Kant, L.~Mihaila and M.~Steinhauser,
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 191602
   [Phys.\ Rev.\ Lett.\  {\bf 101} (2008) 039901]
  [arXiv:0803.0672 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.101.039901, 10.1103/PhysRevLett.100.191602;%%

%32
\bibitem{Kant:2010tf}
  P.~Kant, R.V.~Harlander, L.~Mihaila and M.~Steinhauser,
  JHEP {\bf 1008} (2010) 104
  [arXiv:1005.5709 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2010)104;%%

%33
\bibitem{Harlander:2017kuc}
  R.V.~Harlander, J.~Klappert and A.~Voigt,
  Eur.\ Phys.\ J.\ C {\bf 77} (2017) no.12,  814
  [arXiv:1708.05720 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-5368-6;%%

%34
\bibitem{Jack:1994rk}
  I.~Jack, D.R.T.~Jones, S.P.~Martin, M.T.~Vaughn and Y.~Yamada,
  Phys.\ Rev.\ D {\bf 50} (1994) R5481
  [hep-ph/9407291].
  %%CITATION = doi:10.1103/PhysRevD.50.R5481;%%

%35
\bibitem{Martin:2007pg}
  S.P.~Martin,
  Phys.\ Rev.\ D {\bf 75} (2007) 055005
  [hep-ph/0701051].
  %%CITATION = doi:10.1103/PhysRevD.75.055005;%%

%36
\bibitem{Martin:2014cxa}
  S.P.~Martin and D.G.~Robertson,
  Phys.\ Rev.\ D {\bf 90} (2014) no.7,  073010
  [arXiv:1407.4336 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.073010;%%

%37
\bibitem{Martin:2015eia}
  S.P.~Martin,
  Phys.\ Rev.\ D {\bf 92} (2015) no.5,  054029
  [arXiv:1508.00912 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.054029;%%

%38
\bibitem{Degrassi:2001yf}
  G.~Degrassi, P.~Slavich and F.~Zwirner,
  Nucl.\ Phys.\ B {\bf 611} (2001) 403
  [hep-ph/0105096].
  %%CITATION = doi:10.1016/S0550-3213(01)00343-1;%%

%39
\bibitem{Martin:2001vx}
  S.P.~Martin,
  Phys.\ Rev.\ D {\bf 65} (2002) 116003
  [hep-ph/0111209].
  %%CITATION = doi:10.1103/PhysRevD.65.116003;%%

%40
\bibitem{Martin:2002iu}
  S.P.~Martin,
  Phys.\ Rev.\ D {\bf 66} (2002) 096001
  [hep-ph/0206136].
  %%CITATION = doi:10.1103/PhysRevD.66.096001;%%

%41
\bibitem{Martin:2002wn}
  S.P.~Martin,
  Phys.\ Rev.\ D {\bf 67} (2003) 095012
  [hep-ph/0211366].
  %%CITATION = doi:10.1103/PhysRevD.67.095012;%%

%42
\bibitem{Capper:1979ns}
  D.M.~Capper, D.R.T.~Jones and P.~van Nieuwenhuizen,
  Nucl.\ Phys.\ B {\bf 167} (1980) 479.
  %%CITATION = doi:10.1016/0550-3213(80)90244-8;%%

%43
\bibitem{Stockinger:2005gx}
D.~St\"ockinger
  JHEP {\bf 0503} (2005) 076
[hep-ph/0503129].
%%CITATION = HEP-PH 0503129;%%
%%endref
%%beginref

%45
\bibitem{Harlander:2009mn}
  R.V.~Harlander, L.~Mihaila and M.~Steinhauser,
  Eur.\ Phys.\ J.\ C {\bf 63} (2009) 383
  [arXiv:0905.4807 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-009-1109-9;%%

%46
\bibitem{Harlander:2006xq}
  R.V.~Harlander, D.R.T.~Jones, P.~Kant, L.~Mihaila and M.~Steinhauser,
  JHEP {\bf 0612} (2006) 024
  [hep-ph/0610206].
  %%CITATION = doi:10.1088/1126-6708/2006/12/024;%%

%47
\bibitem{Siegel:1979wq}
  W.~Siegel,
  Phys.\ Lett.\ B {\bf 84} (1979) 193.
  %%CITATION = doi:10.1016/0370-2693(79)90282-X;%%

%48
\bibitem{Bednyakov:2002sf}
  A.~Bednyakov, A.~Onishchenko, V.~Velizhanin and O.~Veretin,
  Eur.\ Phys.\ J.\ C {\bf 29} (2003) 87
  [hep-ph/0210258].
  %%CITATION = doi:10.1140/epjc/s2003-01178-4;%%
%
%
%
%
%

%49
\bibitem{Bednyakov:2005kt}
  A.~Bednyakov, D.I.~Kazakov and A.~Sheplyakov,
  Phys.\ Atom.\ Nucl.\  {\bf 71} (2008) 343
  [hep-ph/0507139].
  %%CITATION = doi:10.1007/s11450-008-2015-6;%%

%50
\bibitem{Martin:1993yx}
  S.P.~Martin and M.~T.~Vaughn,
  Phys.\ Lett.\ B {\bf 318} (1993) 331
  [hep-ph/9308222].
  %%CITATION = doi:10.1016/0370-2693(93)90136-6;%%

%51
\bibitem{Summ:2018oko}
  B.~Summ and A.~Voigt,
  JHEP {\bf 1808} (2018) 026
  [arXiv:1806.05171 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2018)026;%%

%52
\bibitem{h3m}
\href{https://www.ttp.kit.edu/Progdata/ttp10/ttp10-23/}{https://www.ttp.kit.edu/Progdata/ttp10/ttp10-23/}

%53
\bibitem{Hermann:2011ha}
  T.~Hermann, L.~Mihaila and M.~Steinhauser,
  Phys.\ Lett.\ B {\bf 703} (2011) 51
  [arXiv:1106.1060 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2011.07.036;%%

%54
\bibitem{Mathematica}
Wolfram Research, Inc., Mathematica, Version 11.3, Champaign, IL (2018).

%55
\bibitem{Bednyakov:2012en}
  A.V.~Bednyakov, A.F.~Pikelner and V.N.~Velizhanin,
  Phys.\ Lett.\ B {\bf 722} (2013) 336
  [arXiv:1212.6829 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.04.038;%%

%56
\bibitem{Mihaila:2012pz}
  L.N.~Mihaila, J.~Salomon and M.~Steinhauser,
  Phys.\ Rev.\ D {\bf 86} (2012) 096008
  [arXiv:1208.3357 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.096008;%%

%57
\bibitem{Buttazzo:2013uya}
  D.~Buttazzo, G.~Degrassi, P.P.~Giardino, G.F.~Giudice, F.~Sala, A.~Salvio and A.~Strumia,
  JHEP {\bf 1312} (2013) 089
  [arXiv:1307.3536 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2013)089;%%

%58
\bibitem{Bednyakov:2015ooa}
  A.V.~Bednyakov and A.F.~Pikelner,
  Phys.\ Lett.\ B {\bf 762} (2016) 151
  [arXiv:1508.02680 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2016.09.007;%%

%59
\bibitem{Chetyrkin:2016ruf}
  K.G.~Chetyrkin and M.F.~Zoller,
  JHEP {\bf 1606} (2016) 175
  [arXiv:1604.00853 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2016)175;%%

%60
\bibitem{Fanchiotti:1992tu}
  S.~Fanchiotti, B.A.~Kniehl and A.~Sirlin,
  Phys.\ Rev.\ D {\bf 48} (1993) 307
  [hep-ph/9212285].
  %%CITATION = doi:10.1103/PhysRevD.48.307;%%

%61
\bibitem{Chetyrkin:1999qi}
  K.G.~Chetyrkin and M.~Steinhauser,
  Nucl.\ Phys.\ B {\bf 573} (2000) 617
  [hep-ph/9911434].
  %%CITATION = doi:10.1016/S0550-3213(99)00784-1;%%

%62
\bibitem{Melnikov:2000qh}
  K.~Melnikov and T.~van Ritbergen,
  Phys.\ Lett.\ B {\bf 482} (2000) 99
  [hep-ph/9912391].
  %%CITATION = doi:10.1016/S0370-2693(00)00507-4;%%

%63
\bibitem{Chetyrkin:2000yt}
  K.G.~Chetyrkin, J.H.~K\"uhn and M.~Steinhauser,
  Comput.\ Phys.\ Commun.\  {\bf 133} (2000) 43
  [hep-ph/0004189].
  %%CITATION = doi:10.1016/S0010-4655(00)00155-7;%%

%64
\bibitem{Degrassi:2012ry}
  G.~Degrassi, S.~Di Vita, J.~Elias-Miro, J.R.~Espinosa, G.F.~Giudice, G.~Isidori and A.~Strumia,
  JHEP {\bf 1208} (2012) 098
  [arXiv:1205.6497 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2012)098;%%


